LTLf and LDLf Monitoring: A Technical Report

Runtime monitoring is one of the central tasks to provide operational decision support to running business processes, and check on-the-fly whether they comply with constraints and rules. We study runtime monitoring of properties expressed in LTL on finite traces (LTLf) and in its extension LDLf. LDLf is a powerful logic that captures all monadic second order logic on finite traces, which is obtained by combining regular expressions and LTLf, adopting the syntax of propositional dynamic logic (PDL). Interestingly, in spite of its greater expressivity, LDLf has exactly the same computational complexity of LTLf. We show that LDLf is able to capture, in the logic itself, not only the constraints to be monitored, but also the de-facto standard RV-LTL monitors. This makes it possible to declaratively capture monitoring metaconstraints, and check them by relying on usual logical services instead of ad-hoc algorithms. This, in turn, enables to flexibly monitor constraints depending on the monitoring state of other constraints, e.g., "compensation" constraints that are only checked when others are detected to be violated. In addition, we devise a direct translation of LDLf formulas into nondeterministic automata, avoiding to detour to Buechi automata or alternating automata, and we use it to implement a monitoring plug-in for the PROM suite.

==> 2-ldl-old.tex <==
\section{Linear Time Logic and Linear Dynamic Logic on Finite Traces}

In this paper we will adopt the standard \LTL and its variant \LDL interpreted over on finite runs.

\LTL on finite traces, called \LTLf \cite{DegVa13}, has exactly the same syntax as \LTL on infinite traces \cite{Pnueli77}. Namely, given a set of $\Prop$ of propositional symbols, \LTLf formulas are obtained through the following:

\[\varphi ::= a \mid  \ttrue \mid \ffalse \mid \lnot \varphi \mid \varphi_1\land \varphi_2 \mid \varphi_1\lor \varphi_2  \mid \Next\varphi \mid \Wnext\varphi \mid \Diamond\varphi \mid \Box\varphi \mid \varphi_1\Until\varphi_2\]
where $a\in\Prop$ is an atomic proposition in $\Prop$, $\Next$ is the \emph{next} operator, $\Wnext$ is  \emph{weak next}, 
$\Diamond$ is  \emph{eventually}, $\Box$ is  \emph{always}, $\Until$ is  \emph{until}.

The semantics of \LTLf is given in terms of \emph{finite traces} denoting a
finite sequence of consecutive instants of time, i.e., finite words
$\pi$ over the alphabet of $2^\Prop$, containing all possible
propositional interpretations of the propositional symbols in $\Prop$. 
We denote by $\pi(i)$ the $i$th element (or step) in the trace.
We denote by $\pi(i,j)$ the segment of the trace $\pi$ starting at $i$th step end ending at the $j$th step (included). 
%%
Given a finite trace $\pi$, we inductively define when an 
\LTLf formula $\varphi$ \emph{is true} at an step $i$  
(for $1\leq i\leq \last$), written $\pi,i\models\varphi$, as follows:
\begin{compactitem} 
\item $\pi,i\models \ttrue$;
\item $\pi,i\not\models \ffalse$;
\item $\pi,i\models a$, for $a\in\Prop$ ~iff~ $1\leq i \leq \last$ and $a\in\pi(i)$;
\item $\pi,i\models \lnot\varphi$ ~iff~  $\pi,i\not\models\varphi$;
\item $\pi,i\models \varphi_1\land\varphi_2$ ~iff~ $\pi,i\models\varphi_1$ and
  $\pi,i\models\varphi_2$;
\item $\pi,i\models \varphi_1\lor\varphi_2$ ~iff~ $\pi,i\models\varphi_1$ or
  $\pi,i\models\varphi_2$;
\item $\pi,i\models \Next\varphi$ ~iff~ $1\leq i<\last$ and $\pi,i{+}1\models\varphi$;
\item $\pi,i\models \Wnext\varphi$ ~iff~ $1\leq i<\last$ implies $\pi,i{+}1\models\varphi$;
\item $\pi,i\models \Diamond\varphi$ ~iff~ for some $j$ s.t.\ $1\leq i\leq j \leq \last$, we have $\pi,j\models\varphi$;
\item $\pi,i\models \Box\varphi$ ~iff~ for all $j$ s.t.\ $1\leq i\leq j \leq \last$, we have
  $\pi,j\models\varphi$;
\item $\pi,i\models \varphi_1\Until\varphi_2$ ~iff~ for some $j$ s.t.\ $1\leq i\leq j \leq \last$, we have  $\pi,j\models\varphi_2$, and for all $k$, $i\leq k<j$, we have  $\pi,k\models\varphi_1$.
\end{compactitem}
Notice we have the usual boolean equivalences such as $\varphi_1\lor\varphi_2 \equiv \lnot \varphi_1\land \lnot \varphi_2$, furthermore we have that
$\Wnext\varphi \equiv \lnot\Next\lnot\varphi$,
$\Diamond\varphi \equiv \ttrue\Until\varphi$,
$\Box\varphi \equiv \lnot\Diamond\lnot\varphi$.


Notice that the above definition works also if the trace $\pi=\epsilon$ is empty, namely we have:
\begin{compactitem} 
\item $\epsilon,i\models \ttrue$;
\item $\epsilon,i\not\models \ffalse$;
\item $\epsilon,i\not\models a$, for $a\in\Prop$;
\item $\epsilon,i\models \lnot\varphi$ ~iff~  $\epsilon,i\not\models\varphi$;
\item $\epsilon,i\models \varphi_1\land\varphi_2$ ~iff~ $\epsilon,i\models\varphi_1$ and
  $\epsilon,i\models\varphi_2$;
\item $\epsilon,i\models \varphi_1\lor\varphi_2$ ~iff~ $\epsilon,i\models\varphi_1$ or
  $\pi,i\models\varphi_2$;
\item $\epsilon,i\not\models \Next\varphi$;
\item $\epsilon,i\models \Wnext\varphi$;
\item $\epsilon,i\not\models \Diamond\varphi$;
\item $\epsilon,i\models \Box\varphi$;
\item $\epsilon,i\not\models \varphi_1\Until\varphi_2$.
\end{compactitem}

It is known that \LTLf is as expressive as First Order Logic over finite traces, so strictly less expressive than regular expressons which in turn are as expressive as Monadic Second Order logic over finite traces.  On the other hand,  regulare expressions are a too low
level as a formalism for expressing temporal specifications, since, for example, they miss a direct construct for negation and for conjunction \cite{IJCAI13}.

To overcome this difficulties, in \cite{IJCAI13}, 
\emph{Linear Dynamic Logic of Finite Traces}, or \LDLf has been proposed. This logic is as natural as \LTLf but with the full expressive power of Monadic Second Order logic over finite traces.  \LDLf is obtained by merging \LTLf with regular expression through the 
syntax of the well-know logic of programs \PDL, \emph{Propositional Dynamic
Logic}, \cite{FiLa79,Hare84,HaKT00}, but adopting a semantics based
on finite traces.  This logic  is an adaptation of \LDL, introduced in 
\cite{Var11}, which, like \LTL, is interpreted over infinite traces.

Formally, \LDLf formulas are built as follows:
\[\begin{array}{lcl}
\varphi &::=& a \mid \ttrue \mid \ffalse \mid \lnot \varphi \mid \varphi_1 \land \varphi_2 \mid \varphi_1 \land \varphi_2 \mid \DIAM{\rho}\varphi \mid \BOX{\rho}\varphi\\
\rho &::=& \phi \mid \varphi? \mid  \rho_1 + \rho_2 \mid \rho_1; \rho_2 \mid \rho^*
\end{array}
\]
where $a$ is an atomic proposition in $\Prop$;  $\phi$ denotes a propositional formulas over the atomic
propositions in $\Prop$; $\rho$ denotes path expressions, which are
\RE expressions over propositional formulas $\phi$, with the addition of
the test construct $\varphi?$ typical of \PDL; and $\varphi$ stand for \LDLf
formulas built by applying boolean connectives and
the modal connectives $\DIAM{\rho}\varphi$ and $\BOX{\rho}\varphi$.
In fact $\BOX{\rho}\varphi\equiv\lnot\DIAM{\rho}{\lnot\varphi}$.

Intuitively, $\DIAM{\rho}\varphi$ states that, from the current step in the trace,
there exists an execution satisfying the regular expression $\rho$
such that its last step satisfies $\varphi$. While
$\BOX{\rho}\varphi$ states that, from the current step, all
executions satisfying the regular expression $\rho$ are such that
their last step satisfies $\varphi$.

Tests are used to insert into the execution path checks for
satisfaction of additional \LDLf formulas.

 
The semantics of \LDLf is as follows:  an \LDLf formula $\varphi$ \emph{is true} 
at a step $i\in\{1,\ldots,\last\}$, in symbols
$\pi,i\models\varphi$, as follows:
\begin{itemize} 
\item $\pi,i\models \ttrue$
\item $\pi,i\not\models \ffalse$
\item $\pi,i\models a$, for $a\in\Prop$ ~iff~ $1\leq i\leq \last$ and $a\in\pi(i)$.
\item $\pi,i\models \lnot\varphi$ ~iff~ $\pi,i\not\models\varphi$.
\item $\pi,i\models \varphi_1\land\varphi_2$ ~iff~ $\pi,i\models\varphi_1$ and
  $\pi,i\models\varphi_2$.
\item $\pi,i\models \varphi_1\lor\varphi_2$ ~iff~ $\pi,i\models\varphi_1$ or
  $\pi,i\models\varphi_2$.
\item $\pi,i\models \DIAM{\rho}\varphi$ ~iff~  for some $j$ we have
  that $(i,j)\in \R(\rho,\pi(i,\last))$ and $\pi(j,\last)\models\varphi$.
\item $\pi,i\models \BOX{\rho}\varphi$ ~iff~  for all $j$ we have  that $(i,j)\in \R(\rho,\pi(i,\last))$ and $\pi(j,\last)\models\varphi$.
\end{itemize}
The relation $\R(\rho,\pi(i,\last))$ with $1\leq i\leq \last$ is defined inductively as follows:
\begin{itemize}
\item $\R(\phi,\pi(i,\last)) = 
\left \{
\begin{array}{l}
(i,i+1) \;\;\text{if}\; 1\leq i < \last \;\text{and}\; \pi(i)\models \phi\\
\emptyset \;\;\text{if}\; i=\last
\end{array}
\right.
\quad \mbox{($\phi$ propositional)}$
\item $\R(\varphi?,\pi(i,\last) = \{(i,i)\} \;\;\text{if}\;  \pi(i,\last)\models \varphi$
\item $\R(\rho_1+ \rho_2,\pi(i,\last)) = \R(\rho_1,\pi(i,\last))\cup\R(\rho_2,\pi(i,\last))$
\item $\R(\rho_1; \rho_2,\pi(i,\last)) = \{(i,j) \mid \mbox{ exists } k \mbox{  s.t.\  } (i,k)\in\R(\rho_1,\pi(i,\last)) \mbox{ and } (k,j)\in\R(\rho_2,\pi(k,\last))\}$
\item $\R(\rho^*,\pi(i,\last)) = \{(i,i)\}\cup \{(i,j) \mid \mbox{ exists } k \mbox{ s.t.\  } (i,k)\in\R(\rho,\pi(i,\last) \mbox{ and } (k,j)\in\R(\rho^*,\pi(k,\last)\}$
\end{itemize}
Finally, $\R(\rho,\pi(i,\last)) =\emptyset$ if $i>\last$, that is $\pi(i,\last)$ is the empty trace.


It easy to encode \LTLf into  \LDLf: it suffice to observe that we can express the various \LTLf operators by recursively applying the following translations:

\begin{itemize}
\item $\Next \varphi$ translates to $\DIAM{\ttrue} \varphi$
\item $\Wnext \varphi$ translates to $\BOX{\ttrue} \varphi$
\item $\Diamond \phi$ translates to $\DIAM{\ttrue^*} \varphi$
\item $\Box \varphi$ translates to $\BOX{\ttrue^*}\varphi$
\item $\varphi_1  \Until  \varphi_2$ translates to $\DIAM{(\varphi_1?;\ttrue)^*} \varphi_2$
\end{itemize}

It is also easy to encode regular expressions, used as a specification formalism for traces into\LDLf
\begin{itemize}
\item $\rho$ translates to $\DIAM{\rho} \BOX{\ttrue?}\ffalse$
\end{itemize}
Notice that if $\pi, i \not\models \BOX{\ttrue?}\ffalse$ for $1\leq i \leq \last$.
Only if $i>\last$, i.e., the trace $\pi(i,\last)=\epsilon$ is indeed empty  $\pi, i \models \BOX{\ttrue?}\ffalse$ holds.
 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> 3-ldl-automaton-old.tex <==
\section{\LDLf automaton}

We can associate with each \LDLf formula $\varphi$ an (exponential)
\NFA $A_\varphi$ that accepts exactly the traces that make $\varphi$
true.
%%
Here, we provide a simple direct algorithm for computing the \NFA
corresponding to an \LDLf formula.  The correctness of the algorithm
is based on the fact that \myi we can associate with each \LDLf
formula $\varphi$ a polynomial \emph{alternating automaton on words}
(\AFW) $\A_\varphi$ that accept exactly the traces that make $\varphi$
true \cite{DegVa13}, and \myii every \AFW can be transformed into an
\NFA, see, e.g., \cite{DegVa13}. %\cite{BL80,CKS81,Lei81}.
%%
However, to formulate the algorithm we do not need these notions, but
we can work directly on the \LDLf formula.
%%
In order to proceed with the construction of the \AFW $\A_\varphi$, we
put \LDLf formulas $\varphi$ in negation normal form $\nnf(\varphi)$
by exploiting equivalences and pushing negation inside as much as
possible, leaving negations only in front of propositional symbols.
Note that computing $\nnf(\varphi)$ can be done in linear time. In other words, wlog, we consider as syntax for \LDLf the following:

\[\begin{array}{lcl}
\varphi &::=& a \mid \lnot a \mid \ttrue \mid \ffalse \mid (\varphi_1 \land \varphi_2) \mid 
(\varphi_1 \lor \varphi_2) \mid \DIAM{\rho}\varphi \mid \BOX{\rho}\varphi\\
\rho &::=& \phi \mid \varphi? \mid (\rho_1+ \rho_2) \mid 
(\rho_1;\rho_2) \mid (\rho^*).
\end{array}
\]

We assume that all the formulas in $\CL_{\varphi}$ are in negation normal 
form as well.  Also, for convenience, we assume to have a special 
proposition $\Last$ which denotes the last element of the trace.  Note
that $\Last$ can be defined as: $\Last\equiv \BOX{\ttrue}\ffalse$.
%%
%%
Then we define an auxiliary function $\delta$ that takes an \LDLf
formula $\psi$ (in negation normal form) and a propositional
interpretation $\Pi$ for $\Prop$ (including $\Last$), returning a
positive boolean formula whose atoms are (quoted) $\psi$ subformulas.

\[
\begin{array}{lcl}
\delta(\atomize{\ttrue},\Pi) &=& \true\\
\delta(\atomize{\ffalse},\Pi) &=& \false\\
\delta(\atomize{a},\Pi) &=& \true \mbox{ if } a \in \Pi\\
\delta(\atomize{a},\Pi) &=& \false \mbox{ if } a \not\in \Pi\\
%%
\delta(\atomize{\neg a},\Pi) &=& \false \mbox{ if } a \in \Pi\\
\delta(\atomize{\neg a},\Pi) &=& \true \mbox{ if } a \not\in \Pi\\
%%
\delta(\atomize{\varphi_1\land\varphi_2},\Pi) &=& 
\delta(\atomize{\varphi_1},\Pi) \land \delta(\atomize{\varphi_2},\Pi)\\
%%
\delta(\atomize{\varphi_1\lor\varphi_2},\Pi) &=& 
\delta(\atomize{\varphi_1},\Pi) \lor \delta(\atomize{\varphi_2},\Pi)
\end{array}\]
%%
\[\begin{array}{lcl}
\delta(\atomize{\DIAM{\phi}\varphi},\Pi) &=& 
\left\{\hspace{-1ex}\begin{array}{l}
\atomize{\varphi} \mbox{ if } \Last \not \in \Pi \mbox{ and } \Pi \models \phi \quad \mbox{($\phi$  propositional)}\\
\delta(\atomize{\varphi}, \epsilon)  \mbox{ if } \Last \in \Pi \mbox{ and } \Pi \models \phi \\
\false \mbox{ if } \Pi\not\models \phi
\end{array}\right.\\
%%
\delta(\atomize{\DIAM{\psi?}{\varphi}},\Pi) &=& 
\delta(\atomize{\psi},\Pi) \land \delta(\atomize{\varphi},\Pi)\\
%%
\delta(\atomize{\DIAM{\rho_1+\rho_2}{\varphi}},\Pi) &=& 
\delta(\atomize{\DIAM{\rho_1}\varphi},\Pi) \lor \delta(\atomize{\DIAM{\rho_2}\varphi},\Pi)\\
%%
\delta(\atomize{\DIAM{\rho_1;\rho_2}{\varphi}},\Pi) &=& 
\delta(\atomize{\DIAM{\rho_1}\DIAM{\rho_2}\varphi},\Pi)\\
%%
\delta(\atomize{\DIAM{\rho^*}\varphi},\Pi) &=& 
\left\{\hspace{-1ex}\begin{array}{l}
\delta(\atomize{\varphi},\Pi) \hfill \mbox{if  $\rho$ is test-only}\\
\delta(\atomize{\varphi},\Pi) \lor \delta(\atomize{\DIAM{\rho}\DIAM{\rho^*}\varphi},\Pi)
\;\;\hfill  \mbox{o/w}
\end{array}\right.\\
%%
\delta(\atomize{\BOX{\phi}\varphi},\Pi) &=& 
\left\{\hspace{-1ex}\begin{array}{l}
    \atomize{\varphi} \mbox{ if } \Last \not \in \Pi \mbox{ and } \Pi \models \phi \quad \mbox{($\phi$ propositional)}\\
 \delta(\atomize{\varphi},\epsilon) \mbox{ if } \Last \in \Pi \mbox{ and } \Pi \models \phi \quad \mbox{($\phi$ propositional)}\\
    \true \mbox{ if } \Pi\not\models \phi
\end{array}\right.\\
%%
\delta(\atomize{\BOX{\psi?}{\varphi}},\Pi) &=& 
\delta(\atomize{\nnf(\lnot\psi)},\Pi) \lor \delta(\atomize{\varphi},\Pi)\\
%%
\delta(\atomize{\BOX{\rho_1+\rho_2}{\varphi}},\Pi) &=& 
\delta(\atomize{\BOX{\rho_1}\varphi},\Pi)\land\delta(\atomize{\BOX{\rho_2}\varphi},\Pi)\\
%%
\delta(\atomize{\BOX{\rho_1;\rho_2}{\varphi}},\Pi) &=& 
\delta(\atomize{\BOX{\rho_1}\BOX{\rho_2}\varphi},\Pi)\\
%%
\delta(\atomize{\BOX{\rho^*}\varphi},\Pi) &=& 
\left\{\hspace{-1ex}
\begin{array}{ll}
\delta(\atomize{\varphi},\Pi) \hfill \mbox{if  $\rho$ is test-only}\\
\delta(\atomize{\varphi},\Pi) \land \delta(\atomize{\BOX{\rho}\BOX{\rho^*}\varphi},\Pi) 
\;\;\hfill \mbox{o/w}
\end{array}\right.
\end{array}
\]
where $\delta(\atomize{\varphi},\epsilon)$, i.e., the interpretation of \LDLf formula in the case the (remaining fragment of the) trace is empty, is defined as follows:
\[
\begin{array}{lcl}
\delta(\atomize{\ttrue},\epsilon) &=& \true\\
\delta(\atomize{\ffalse},\epsilon) &=& \false\\
\delta(\atomize{a},\epsilon) &=& \false\\
\delta(\atomize{\neg a},\epsilon) &=& \false\\
%%
\delta(\atomize{\varphi_1\land\varphi_2},\epsilon) &=& 
\delta(\atomize{\varphi_1},\epsilon) \land \delta(\atomize{\varphi_2},\epsilon)\\
%%
\delta(\atomize{\varphi_1\lor\varphi_2},\epsilon) &=& 
\delta(\atomize{\varphi_1},\epsilon) \lor \delta(\atomize{\varphi_2},\epsilon)\\
%%
% \delta(\atomize{\DIAM{\rho}\varphi},\epsilon) &=& \false\\
% %%
% \delta(\atomize{\BOX{\rho}\varphi},\epsilon) &=& \true
%
\delta(\atomize{\DIAM{\phi}\varphi},\epsilon) &=& \false \quad \mbox{($\phi$  propositional)}\\
%%
\delta(\atomize{\DIAM{\psi?}{\varphi}},\epsilon) &=& \false\\
~%\delta(\atomize{\psi},\epsilon) \land \delta(\atomize{\varphi},\epsilon)\\
%%
\delta(\atomize{\DIAM{\rho_1+\rho_2}{\varphi}},\epsilon) &=& 
\delta(\atomize{\DIAM{\rho_1}\varphi},\epsilon) \lor \delta(\atomize{\DIAM{\rho_2}\varphi},\epsilon)\\
%%
\delta(\atomize{\DIAM{\rho_1;\rho_2}{\varphi}},\epsilon) &=& 
\delta(\atomize{\DIAM{\rho_1}\DIAM{\rho_2}\varphi},\epsilon)\\
%%
\delta(\atomize{\DIAM{\rho^*}\varphi},\epsilon) &=& \delta(\atomize{\varphi},\epsilon)\\
%%\left\{\hspace{-1ex}\begin{array}{l}
%%\delta(\atomize{\varphi},\epsilon)
%% \hfill \mbox{if  $\rho$ is test-only}\\
%%\delta(\atomize{\varphi},\epsilon) \lor \delta(\atomize{\DIAM{\rho}\DIAM{\rho^*}\varphi},\epsilon) \;\;\hfill  \mbox{o/w}
%%\end{array}\right.\\
%%
\delta(\atomize{\BOX{\phi}\varphi},\epsilon) &=& \true \quad \mbox{($\phi$ propositional)}\\
%%
\delta(\atomize{\BOX{\psi?}{\varphi}},\epsilon) &=& \true\\
%%\delta(\atomize{\nnf(\lnot\psi)},\epsilon) \lor \delta(\atomize{\varphi},\epsilon)\\
%%
\delta(\atomize{\BOX{\rho_1+\rho_2}{\varphi}},\epsilon) &=& 
\delta(\atomize{\BOX{\rho_1}\varphi},\epsilon)\land\delta(\atomize{\BOX{\rho_2}\varphi},\epsilon)\\
%%
\delta(\atomize{\BOX{\rho_1;\rho_2}{\varphi}},\epsilon) &=& 
\delta(\atomize{\BOX{\rho_1}\BOX{\rho_2}\varphi},\epsilon)\\
%%
\delta(\atomize{\BOX{\rho^*}\varphi},\epsilon) &=& \delta(\atomize{\varphi},\epsilon)\\
% \left\{\hspace{-1ex}
% \begin{array}{ll}
% \delta(\atomize{\varphi},\epsilon) \hfill \mbox{if  $\rho$ is test-only}\\
% \delta(\atomize{\varphi},\epsilon) \land \delta(\atomize{\BOX{\rho}\BOX{\rho^*}\varphi},\epsilon) 
% \;\;\hfill \mbox{o/w}
% \end{array}\right.
\end{array}
\]


\noindent Using the auxiliary function $\delta$ we can build the \NFA
$A_\varphi$ of an \LTLf formula $\varphi$ in a forward fashion.
States of $A_\varphi$ are sets of atoms (recall that each atom is
quoted $\varphi$ subformulas) to be interpreted as a conjunction; the
empty conjunction $\emptyset$ stands for $\true$:
% as shown in Figure~\ref{fig:algo}.

\newcommand{\algoname}{\textsc{{\LDLf}2\NFA}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\algrenewcommand\algorithmicindent{1em}

% \begin{figure}[!t]
\begin{algorithmic}[1]
  \small \State\textbf{algorithm} \algoname() \\\textbf{input} \LTLf
  formula $\varphi$ \\\textbf{output} \NFA $A_\varphi =
  (2^\Prop,\S,\{s_0\},\varrho,\{s_f\})$ \State $s_0 \gets
  \{\atomize{\varphi}\}$ \Comment{single initial state} \State $s_f
  \gets \emptyset$ \Comment{single final state} \State $\S \gets
  \{s_0,s_f\}$, $\varrho \gets \emptyset$ \While{($\S$ or $\varrho$
    change)} %\{
  \If{($q\in \S$ and $q'\models \bigwedge_{(\atomize{\psi}\in q)}
    \delta(\atomize{\psi},\Pi)$)}

  \State $\S \gets \S \cup \{q'\}$ \Comment{update set of states}
  \State $\varrho \gets \varrho \cup \{ (q,\Pi,q')\}$ \Comment{update
    transition relation}
  \EndIf
  \EndWhile
  % \State \}
  % \EndFunction
  % \noindent
\end{algorithmic}
% \vspace{-.3cm}
% \caption{\NFA construction }\label{alg:ts}
% \end{figure}
where $q'$ is a set of quoted subformulas of $\varphi$ that denotes a
minimal interpretation such that $q'\models
\bigwedge_{(\atomize{\psi}\in q)} \delta(\atomize{\psi},\Pi)$. (Note:
we do not need to get all $q$ such that $q'\models
\bigwedge_{(\atomize{\psi}\in q)} \delta(\atomize{\psi},\Pi)$, but
only the minimal ones.)  Notice that trivially we have
$(\emptyset,a,\emptyset)\in\varrho$ for every $a\in\Sigma$.
%%
\begin{comment}
  \begin{figure}[!t]
    \begin{algorithmic}[1]
      \small \Function{build-\NFA}{} \\\textbf{input} \LDLf formula
      $\varphi$ \\\textbf{output} \NFA $A_\varphi =
      (2^\Prop,S,s^0,\rho,\F)$ \State $s^0 \gets \varphi$
      % \Comment{Single initial state}
      \State $\F\gets \{\true,\final\} \mbox{ ($\true$ stands for
        $\emptyset$ -- empty set of atoms)}$
      % \Comment{Single final state}
      \State $ S \gets \{s^0,s^f,\final\}$, $\rho \gets \emptyset$
      \While{($S$ or $\rho$ change)} %\{
      \If{($T\in S$ and $T'\models \bigwedge_{t\in T} \delta(t,\Pi)$)}

      \State $S \gets S \cup \{T'\}$ \Comment{update set of states}
      \State $\rho \gets \rho \cup (T,\Pi,T')$ \Comment{update
        transition relation}
      \EndIf
      \EndWhile
      % \State \}
      \EndFunction

      \medskip
      \noindent
      where $T'$ is a conjunction of formulas (considered as atoms) in
      the Fisher-Ladner closure $\CL(\varphi)$. Note: we do not need
      to get all $T'$ such that $T'\models \bigwedge_{t\in T}
      \delta(t,\Pi)$, but only the minimal ones.  Notice that
      trivially we have $(\true,a,\true)\in\rho$ for every
      $a\in\Sigma$.
    \end{algorithmic}
    \vspace{-.3cm}
    \caption{\NFA construction }\label{alg:ts}
  \end{figure}
\end{comment}
%%

The algorithm \algoname\ terminates in at most exponential number of
steps, and generates a set of states $\S$ whose size is at most
exponential in the size of the formula $\varphi$.

\begin{theorem}
  Let $\varphi$ be an \LDLf formula and $A_\varphi$ the \NFA
  constructed as above. Then $\pi\models\varphi \mbox{ iff } \pi\in
  L(A_\varphi)$ for every finite trace $\pi$.
\end{theorem}
\begin{proofsk}
  Given a specific formula $\varphi$, $\delta$ grounded on the
  subformulas of $\varphi$ becomes the transition function of the
  \AFW, with initial state $\atomize{\varphi}$ and no final states,
  corresponding to $\varphi$ \cite{DegVa13}. Then \algoname\
  essentially transforms the \AFW into a \NFA.
\end{proofsk}
% \begin{comment}
%   \begin{end}
%     We recall that the general construction \cite{BL80,CKS81,Lei81}
%     for transforming an \AFW $\A=(\Sigma,\S,s^0,\delta,\F)$ into an
%     \NFA $A=(\Sigma, S, S^0,\rho,F)$, is as follows: \myi $S=2^\S$,
%     each element in $S$ should be intended as a conjunction (notice
%     that $\emptyset$ stands for the empty conjunction denoting
%     $\true$); \myii $S^0=\{s^0\}$; \myiii $F= 2^\F$; \myiv
%     $(T,a,T')\in\rho$ if $T'\models \bigwedge_{t\in T} \delta(t,a)$.
%     Intuitively, \NFA $A$ guesses a run tree of \AFW $\A$. At a given
%     point of a run of \NFA $A$ , it keeps in its memory a whole level
%     of the run tree of \AFW $\A$. As the \NFA $A$ reads the next input
%     symbol, it guesses the next level of the run tree of \AFW $\A$.

%     In our case, since the initial state of the \AFW for the \LTLf
%     formula $\varphi$ is $\varphi$, the initial state of the \NFA is
%     $S^0_n = \{\varphi\}$. A
% %%
%     And since the set of final states of the \AFW is $\F=\emptyset$,
%     the final state (only one!) of the \NFA is $F_n=2^\emptyset=
%     \{\emptyset\}$.
% %%
%     The algorithm applies the general construction on-the-fly in a
%     forward fashion.
%   \end{proof}
% \end{comment}



Notice that above we have assumed to have a special proposition
$\Last\in\Prop$.  If we want to remove such an assumption, we can
easily transform the obtained automaton $A_\varphi =
(2^\Prop,\S,\{\atomize{\varphi}\},\varrho,\{\emptyset\})$ into the new
automaton
\[A'_\varphi =
(2^{\Prop-\{\Last\}},\S\cup\{\textit{ended}\},\{\atomize{\varphi}\},\varrho',\{\emptyset,
\textit{ended}\})\] where:
% \begin{inparaenum}[\it (i)]
% \item $\Prop' = \Prop - \{\Last\}$;
% \item $\S'_0 = \{s_0\}$;
% \item $S' = S \cup \{\textit{ended}\}$;
% \item $S'_f = \{true, \textit{ended}\}$;
% \item
$(q, \Pi', q') \in \varrho'$ iff $(q, \Pi', q')\in\varrho$, or $(q,
\Pi'\cup\{\Last\}, \true) \in \varrho$ and $q'=\textit{ended}$.
% \end{inparaenum}

It is easy to see that the \NFA obtained can be built on-the-fly while
checking for nonemptiness, hence we have:
\begin{theorem}
  Satisfiability of an \LDLf formula can be checked in PSPACE by
  nonemptiness of $A_\varphi$ (or $A'_\varphi$).
\end{theorem}
Considering that it is known that satisfiability in \LDLf is a PSPACE-complete problem we can conclude that the proposed construction is optimal wrt computational
complexity for satisfiability (as well as for validity and logical implication which are linearly reducible to satisfiability in \LDLf) c.f. \cite{IJCAI13}.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> 6-conditional-monitoring.tex <==
\section{Conditional \LDLf monitoring}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> 7-related-work.tex <==
\section{Related work}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

==> declare-table_copy.tex <==


\newcommand{\ot}{o}

\begin{table*}[t!]
\caption{\label{tab:constraints}Declare patterns and their
  insensitivity to infiniteness}
\scalebox{0.7}{
\begin{tabularx}{1.43\textwidth}{@{}c@{\ }l@{\ }l@{\ } l @{\ } l@{\ }X@{}}
\toprule
& \textsc{name} & \textsc{notation} & $\pref$ &  $\bpref$ & \textsc{possible states}\\
\midrule
%\multicolumn{5}{@{}l@{}}{\textsc{existence patterns}}\\
%\midrule
\parbox[b]{4mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{existence\!\!\!\!}}}}
&
\textbf{Existence} 
&
\existenceformula{\existenceN{1}}{a}
&
$(a+\ot)^*$
&
$\emptyset$
&
$\tempfalse$, $\true$
\\
\cmidrule{2-6}
&
\textbf{Absence 2} 
&
\existenceformula{\absenceN{1}}{a}
&
$\ot^*+(\ot^*;a;\ot^*)$
&
$\ot^*;a;\ot^*;a;(\ot+a)^*$
&
$\temptrue$, $\false$
\\
\midrule
\parbox[b]{4mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{choice}}}}
&
\textbf{Choice} 
&
\relationformula{\choice}{a}{b} 
&
$(a+b+\ot)^*$
&
$\emptyset$
&
$\tempfalse$, $\true$
\\
\cmidrule{2-6}
&
\textbf{Exclusive Choice}
&
\relationformula{\exclusivechoice}{a}{b}
&
$(a+\ot)^*+(b+\ot)^*$
&
$
\begin{array}{@{}l@{}}
\ot^*+(\ot^*;a;(a+\ot)^*;b;(a+b+\ot)^*)\\
+(\ot^*;b;(b+\ot)^*;a;(a+b+\ot)^*)
\end{array}
$
&
$\tempfalse$, $\temptrue$, $\false$
\\
\midrule
%\multicolumn{5}{@{}l@{}}{\textsc{relation patterns}}\\
%\midrule
\parbox[b]{4mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{\textsc{relation}}}}
&
\textbf{Resp.\ existence} 
&
\relationformula{\respondedexistence}{a}{b}
&
$(a+b+\ot)^*$
&
$\emptyset$
&
$\temptrue$, $\tempfalse$, $\true$
\\
\cmidrule{2-6}
&
\textbf{Coexistence} 
&
\relationformula{\coexistence}{a}{b}
&
$(a+b+\ot)^*$
&
$\emptyset$
&
$\temptrue$, $\tempfalse$, $\true$
\\
\cmidrule{2-6}
&
\textbf{Response} 
&
\relationformula{\response}{a}{b}
&
$(a+b+\ot)^*$
&
$\emptyset$
&
$\temptrue$, $\tempfalse$
\\
\cmidrule{2-6}
&
\textbf{Precedence} 
&
\relationformula{\precedence}{a}{b}
&
$\ot^*;(a;(a+b+\ot)^*)^*$
&
$\ot^*;b;(a+b+\ot)^*$
&
$\temptrue$, $\true$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Succession} 
&
\relationformula{\succession}{a}{b}
&
$\ot^*;(a;(a+b+\ot)^*)^*$
&
$\ot^*;b;(a+b+\ot)^*$
&
$\temptrue$, $\tempfalse$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Alt.\ Response} 
&
\relationformula{\alternateresponse}{a}{b}
&
$((b+\ot)^*;(a;\ot^*;b)^*)^*$
&
$(b+\ot)^*;a;\ot^*;a;(a+b+\ot)^*$
&
$\temptrue$, $\tempfalse$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Alt.\ Precedence} 
&
\relationformula{\alternateprecedence}{a}{b}
&
$\ot^*;(a;(a+\ot)^*;(a+b+\ot))^*$
&
$\begin{array}{@{}l@{}}
 (\ot^*;b;(a+b+\ot)^*)
\\+((a+\ot)^*;b;\ot^*;b;(a+b+\ot)^*)
\end{array}
$
&
$\temptrue$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Alt.\ Succession} 
&
\relationformula{\alternatesuccession}{a}{b}
&
$\ot^*;(a;\ot^*;b;\ot^*)^*$
&
$
\begin{array}{@{}l@{}}
(b+\ot)^*;a;\ot^*;a;(a+b+\ot)^*\\
+ (\ot^*;b;(a+b+\ot)^*)\\
+((a+\ot)^*;b;\ot^*;b;(a+b+\ot)^*)
\end{array}
$
&
$\temptrue$, $\tempfalse$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Chain Response} 
&
\relationformula{\chainresponse}{a}{b}
&
$(b+\ot)^*;(a;b;\ot^*)^*$
&
$(b+\ot)^*;a;(a+\ot);(a+b+\ot)^*$
&
$\temptrue$, $\tempfalse$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Chain Precedence} 
&
\relationformula{\chainprecedence}{a}{b}
&
%$(\ot+a)^*;(a;(b+\epsilon);\ot)^*$
$(a+\ot)^*+((a+\ot)^*;a;b)^*$
&
$
(a+\ot)^*;(b+\ot);b;(a+b+\ot)^*
$
&
$\temptrue$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Chain Succession} 
&
\relationformula{\chainsuccession}{a}{b}
&
$\ot^*;(a;b;\ot^*)^*$
&
$
\begin{array}{@{}l@{}}
((a+\ot)^*;(b+\ot);b;(a+b+\ot)^*)\\
+((b+\ot)^*;a;(a+\ot);(a+b+\ot)^*)
\end{array}
$
&
$\temptrue$, $\tempfalse$, $\false$
\\
%\cmidrule{2-6}
%\multicolumn{5}{@{}l@{}}{\textsc{negation patterns}}\\
\midrule
\parbox[b]{4mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textsc{negation}}}}
&
\textbf{Not Coexistence} 
&
\negationformula{\coexistence}{a}{b}
&
$(a+\ot)^*+(b+\ot)^*$
&
$
\begin{array}{@{}l@{}}
(\ot^*;a;(a+\ot)^*;b;(a+b+\ot)^*)\\
+(\ot^*;b;(b+\ot)^*;a;(a+b+\ot)^*)
\end{array}
$
&
$\temptrue$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Neg.\ Succession} 
&
\negationformula{\succession}{a}{b}
&
$(b+\ot)^*;(a+\ot)^*$
&
$(b+\ot)^*;a;(a+\ot)^*;b;(a+b+\ot)^*$
&
$\temptrue$, $\false$
\\
\cmidrule{2-6}
&
\textbf{Neg.\ Chain Succ.} 
&
\negationformula{\chainsuccession}{a}{b}
&
$((b+\ot)^*;(a;\ot)^*)^*$
&
$(b+\ot)^*;a;b;(a+b+\ot)^*$
&
$\temptrue$, $\false$
\\
\bottomrule
\end{tabularx}
}
\end{table*}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

